On weighted uncertainty sampling in active learning

This note explores probabilistic sampling weighted by uncertainty in active learning. This method has been previously used and authors have tangentially remarked on its efficacy. The scheme has several benefits: (1) it is computationally cheap, (2) it can be implemented in a single-pass streaming fashion which is a benefit when deployed in real-world systems where different subsystems perform the suggestion scoring and extraction of user feedback, and (3) it is easily parameterizable. In this paper, we show on publicly available datasets that using probabilistic weighting is often beneficial and strikes a good compromise between exploration and representation especially when the starting set of labelled points is biased.

==> related_work.tex <==
\section{Related work}
\label{sec:related_work}
\subsection{Active Learning}
\label{sec:active_learning_background}
Classic approaches such as uncertainty-based sampling~\cite{settles2012active}, query by committee~\cite{Seung1992queryByCommittee}, expected error change~\cite{settles2008multiple}, expected variance reduction~\cite{zhang2000value}, expected error reduction~\cite{zhu2003combining} focus on identifying and querying "informative" samples for the trained classifier and consequently, explore the {\em known unknowns}~\cite{attenberg2011beat}.

On the other hand, methods which query based on "representativeness" such as clustering

Two recent works~\cite{du2017exploring,lakkaraju2017identifying} have presented methods to address the informativeness versus representativeness trade-off. \citet{du2017exploring} present a QP-based approach which ... 
\citet{lakkaraju2017identifying} have present a method for identifying the {\em unknown unknowns} in a black-box setting, where the underlying data is not available directly rather only distances between points can be obtained. 

\subsection{Prevalence Estimation}
\label{sec:prevalence_estimation_background}

\subsection{Crowdsourcing}
\label{sec:crowdsourcing_background}

\subsection{Active Relabeling}
\label{sec:active_relabeling_background}

